An ACA Survey of [CI] $^3P_1-^3P_0$, CO $J=4-3$, and Dust Continuum in Nearby U/LIRG

We present the results of surveying [CI] $^3P_1-^3P_0$, $^{12}$CO $J=4-3$, and 630 $\mu$m dust continuum emission for 36 nearby ultra/luminous infrared galaxies (U/LIRGs) using the Band 8 receiver mounted on the Atacama Compact Array (ACA) of the Atacama Large Millimeter/submillimeter Array. We describe the survey, observations, data reduction, and results; the main results are as follows. (i) We confirmed that [CI] $^3P_1-^3P_0$ has a linear relationship with both the $^{12}$CO $J=4-3$and 630 $\mu$m continuum. (ii) In NGC 6052 and NGC 7679, $^{12}$CO $J=4-3$ was detected but [CI] $^3P_1-^3P_0$ was not detected with a [CI] $^3P_1-^3P_0$/ $^{12}$CO $J=4-3$ ratio of $\lesssim0.08$. Two possible scenarios of weak [CI] $^3P_1-^3P_0$ emission are C$^0$-poor/CO-rich environments or an environment with an extremely large [CI] $^3P_1-^3P_0$ missing flux. (iii) There is no clear evidence showing that galaxy mergers, AGNs, and dust temperatures control the ratios of [CI] $^3P_1-^3P_0$/ $^{12}$CO $J=4-3$ and $L'_{\rm [CI](1-0)}/L_{\rm 630\mu m}$. (iv) We compare our nearby U/LIRGs with high-z galaxies, such as galaxies on the star formation main sequence (MS) at z$\sim1$ and submillimeter galaxies (SMGs) at $z=2-4$. We found that the mean value for the [CII] $^3P_1$--$^3P_0$/ $^{12}$CO $J=4-3$ ratio of U/LIRGs is similar to that of SMGs but smaller than that of galaxies on the MS.

==> DSS_FigSet.tex <==
\begin{figure}[!htbp]\label{fig:SED}
\figurenum{A1.1}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_1.png}
\caption{The optical image obtained by Digitized Sky Survey (DSS), the fits images are obtained by astroquery.skyview modules in Python. The magenta circle indicates the [C I](1–0) FoV.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.2}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_2.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}


\begin{figure}[!htbp]
\figurenum{A1.3}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_3.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.4}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_4.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.5}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_5.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.6}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_6.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.7}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_7.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.8}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_8.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.9}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_9.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.10}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_10.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.11}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_11.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.12}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_12.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.13}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_13.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.14}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_14.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\figurenum{A1.15}
\begin{center}
\includegraphics[angle=0,scale=0.5]{f1_15.png}
\caption{Same as Figure A1.1.}
\end{center}
\end{figure}




==> R_GD_CO10.tex <==
20 and 100

==> mom_FigSet.tex <==

\clearpage
\begin{figure*}[!htbp]\label{fig:mom}
\figurenum{A2.1}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_1.png}
\caption{(a) The velocity integrated intensity map (mom0) of [\ion{C}{1}]~(1--0) emission line. The $n$th contours are at $3n\sigma$ where $\sigma$ is the rms revel of the map shown in Table~\ref{tab:obs_res}. The magenta circle indicates the ACA FoV calculated by equation~\ref{eq:FoV}.
(b) The velocity field map (mom1) of [\ion{C}{1}]~(1--0) emission line.
(c) The velocity dispersion map (mom2) of [\ion{C}{1}]~(1--0) emission line.
The mom1 and mom2 maps are made by clipping 3$\sigma$ emission in data cube.
(d) The continuum emission map associated with [\ion{C}{1}]~(1--0) observation. The $n$th contours are at $3n\sigma$ where $\sigma$ is the rms revel of the map shown in Table~\ref{tab:obs_res}. 
(e)-(h) The same map with (a)-(d) but for CO~(4--3) emission.  
(i) and (j) The CO~(4--3) and [\ion{C}{1}]~(1--0) spectrum with the aperture of FoV.
The spectrum were derived from ${\tt specflux}$ task in ${\tt CASA}$.
(k) The normalized CO~(4--3) and [\ion{C}{1}]~(1--0) spectrum. The velocity is calculated as the offset from the systematic velocity shown in Table~\ref{tab:target}.
In the case of CO~(4--3) detection and [\ion{C}{1}]~(1--0) non-detection,  [\ion{C}{1}]~(1--0) moment maps are made by assuming same velocity range for integration.
If both CO~(4--3) and [\ion{C}{1}]~(1--0) are non-detection, we integrated $\pm200$~km~s$^{-1}$ from systematic velocities.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.2}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_2.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.3}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_3.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.4}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_4.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.5}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_5.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.6}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_6.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.7}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_7.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.8}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_8.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.9}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_9.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.10}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_10.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.11}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_11.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.12}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_12.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}


\begin{figure*}[!htbp]
\figurenum{A2.13}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_13.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.14}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_14.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.15}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_15.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.16}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_16.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.17}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_17.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.18}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_18.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.19}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_19.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.20}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_20.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.21}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_21.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.22}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_22.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.23}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_23.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.24}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_24.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.25}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_25.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.26}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_26.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.27}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_27.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.28}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_28.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.29}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_29.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.30}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_30.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.31}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_31.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.32}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_32.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.33}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_33.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.34}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_34.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.35}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_35.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.36}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_36.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.37}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_37.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.38}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_38.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.39}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_39.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}

\begin{figure*}[!htbp]
\figurenum{A2.40}
\begin{center}
\includegraphics[angle=0,scale=0.4]{f2_40.png}
\caption{Same as Figure A2.1.}
\end{center}
\end{figure*}










